Code Search: A Survey of Techniques for Finding Code

The immense amounts of source code provide ample challenges and opportunities during software development. To handle the size of code bases, developers commonly search for code, e.g., when trying to find where a particular feature is implemented or when looking for code examples to reuse. To support developers in finding relevant code, various code search engines have been proposed. This article surveys 30 years of research on code search, giving a comprehensive overview of challenges and techniques that address them. We discuss the kinds of queries that code search engines support, how to preprocess and expand queries, different techniques for indexing and retrieving code, and ways to rank and prune search results. Moreover, we describe empirical studies of code search in practice. Based on the discussion of prior work, we conclude the article with an outline of challenges and opportunities to be addressed in the future.

==> sections/codepreprocessing.tex <==
\section{Preprocessing and Abstraction of Code}
\label{sec:codepre}












==> sections/feature.tex <==
\section{Feature Extraction}

==> sections/indexingmatching.tex <==
\section{Indexing and Matching}

==> sections/methodology.tex <==
\section{Survey Methodology}

==> sections/pruning.tex <==
\section{Final Pruning}

==> sections/random.tex <==
\section{Papers that don't fit any other section}

\subsection{\citet{Gallardo-Valencia2009}}
This paper presents the general problem of Internet-Scale Code Search, that recently increased thanks to the increment of open source code available online. They compare this new challenge with the techniques used in code search, information retrieval, software reuse, and program comprehension.

